Translating Behavioral Theory into Technological Interventions: Case Study of an mHealth App to Increase Self-reporting of Substance-Use Related Data

Mobile health (mHealth) applications are a powerful medium for providing behavioral interventions, and systematic reviews suggest that theory-based interventions are more effective. However, how exactly theoretical concepts should be translated into features of technological interventions is often not clear. There is a gulf between the abstract nature of psychological theory and the concreteness of the designs needed to build health technologies. In this paper, we use SARA, a mobile app we developed to support substance-use research among adolescents and young adults, as a case study of a process of translating behavioral theory into mHealth intervention design. SARA was designed to increase adherence to daily self-report in longitudinal epidemiological studies. To achieve this goal, we implemented a number of constructs from the operant conditioning theory. We describe our design process and discuss how we operationalized theoretical constructs in the light of design constraints, user feedback, and empirical data from four formative studies.

==> 3-related-discussion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% MASH TO PEDJA --- Following two sections are new. I wrote a new related work and limitation section
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{\textbf{Limitations of the SARA design and evaluation}}
We finish our discussion of the iterative design of SARA with a set of limitations. These limitations are additional constraints that affected how we designed SARA and ran the evaluation studies.\\


\noindent
As part of our design process, we did not consider the growing literature on personal informatics in HCI ~\cite{li2010stage,epstein2015lived,schwanda2011side,cordeiro2015barriers,clawson2015no,epstein2016beyond,lazar2015we,gouveia2015we,patel2015contextual,baumer2013limiting}. Personal informatics largely deals with health and other behaviors that are already meaningful to end users. SARA, on the other hand, targets self-reporting behavior in the context of a research study. It is not clear that self-reporting is personally meaningful to AYA substance users with low problem severity (e.g., recent binge drinking or marijuana use) who are enrolled in EMA studies examining daily factors associated with use~\cite{wray2014using}. As such, it is unclear to what extent the findings from the literature on personal informatics are applicable to self-reporting as target behavior.\\


%for three reasons: (\underline{\textbf{i}}) although personal informatics literature frequently advocates goal-setting, self-reflection and journaling for behavior change, there is  lack consensus on what strategy to use when~\cite{ayobi2016reflections,zuckerman2014deconstructing,gulotta2016fostering,ayobi2018reflections}.For example, Gulotta et al.~\cite{gulotta2016fostering} argue for goal setting over self-reflection or journaling, while Meng et al.~\cite{info:doi/10.2196/10139} suggest that patients prefer self-reflection but caregivers prefer goal-setting in a student mental health care facility. Thus, we chose to wait for the personal informatics literature to mature, because, as we demonstrated, theory translation is difficult even for a well-specified theory like OCT. (\underline{\textbf{ii}}) people interested in goal-setting, self-reflection or journaling are already highly motivated. Some of these people are quantified selfers who are more healthy and self-conscious than the average person. In contrast, SARA  tries to engage new users who are also AYA substance users and likely more reluctant to engage~\cite{hoeppner2017there,kazemi2017systematic,majeed2015apps,lenhart2015smartphones,chan2017adolescents}. (\underline{\textbf{iii}}) journaling, goal-setting or self-reflection consider therapeutic benefits (i.e., improving substance use behavior) as a mechanism of user engagement. However, the downstream effects of goal setting or self-reflection are unclear for AYA substance use; e.g., only one study tried goal setting for cannibis use in a non mobile health setting~\cite{lozano2006abstinence,spinola2017motivation}, and self-reflection can increase shame, which may lead to substance use in AYA~\cite{rahim2015association,reimer1996sinking,velotti2014shame,brown2009shame}. Nonetheless, SARA is an extendable app, and future versions can test personal informatics strategies in the same way that we randomized memes and life-insights in iteration 4 (Section 3.6) ~\cite{finn1997information,rabbisaint}.\\ 

\noindent
Another limitation is that the 30-day study we conducted used a single-arm design (Section 3.10). One could question whether this duration is long enough to test the adherence interventions we designed and, lacking a control arm, how much confidence we can have in our results. We chose the 30-day study length because it is a typical length for many observational substance use studies~\cite{suffoletto2012text,shrier2018pilot,clark2010project}. This period is also sufficient to examine engagement, as compliance with daily assessments declines over 30 days in samples of substance-using youth~\cite{bonar2018feasibility,buu2017assessment,comulada2015compliance,suffoletto2012text,wen2017compliance}. Thus, a 30-day study was an efficient way to iterate on our design decisions while keeping the study duration in line with other research in this area.\\

\noindent
We did not use a control arm because the goal of this study was optimization, rather than a confirmatory evaluation. Specifically, our study was intended to generate data that would allow us to create predictors of disengagement and add more incentives that tackle those points of disengagement. Such optimization trials are often advocated as efficient ways of improving interventions prior to conducting expensive randomized controlled trials~\cite{collins2018optimization}.
Finally, beyond a misalignment with the optimization goals of the study, conducting an RCT would have made the study less feasible. Recruitment for the current single-arm study was already quite demanding. We recruited participants from an emergency department of a North American medical facility where other substance use studies were running at the same time. Our recruiters had to work 6PM-midnight shifts  3-5 days a week to find eligible participants. The recruitment rate was still slow, and it took us four months to recruit the 37 people for User Study 4 (section 3.10). Thus, due to these real-world constraints, for the purposes of this formative evaluation, we compared SARA's adherence rate to similar AYA substance use studies~\cite{bonar2018feasibility}.\\

\noindent
{\color{blue} Finally, we only reported overall the adherence rates of SARA in the user study in section 3.10. One reason is that overall adherence rate is the most important metric of how SARA will improve self-report adherence. However, we did not report the effect of individual interventions (such as fish, meme or life-insights), because the effects of individual interventions are part of the primary analyses of the clinical trial,  from which user study 4 participants are drawn [X]\footnote{anonymized for review}. We cannot pre-analyze the effect of individual interventions, because doing so would cause p-value hacking issues for the clinical trial. Also, the results of clinical trials are better suited for non-technical behavior science journals, where these results will be published by our behavioral science collaborators who gave us access to the high-risk AYA substance use population.}





%The emerging mechanisms of change in personal informatics literature are goal setting, self-reflection, and journaling. Although personal informatics literature deals with technological design, 
%We first discuss related work on theory translation. Since the SARA app itself is a secondary contribution to this paper, we also discuss related works on increasing self-report adherence.\\
%The final limitation is that we did not provide any intervention to improve substance use behaviors. As we have explained, SARA, like many substance use studies, is observational in nature~\cite{suffoletto2012text,shrier2018pilot,clark2010project}. Furthermore, AYA substance use behavior is  poorly understood, so there is a lack of knowledge about what is a good predictor for substance use. The data from the first SARA trial will provide valuable information on what are good predictors of substance use, and we will provide substance use interventions in future versions of SARA.
%\textbf{Translating theory into technological interventions:}
%--- talk about in the HCI literature the topic of theory translation has not been talked about. 
%Hekler et al.'s~\cite{hekler2013mind} \textit{Mind the theoretical gap} paper discussed several gaps between behavioral theories and current HCI design practices. One of the gaps is related to  theory translation. Hekler et al. used a hypothetical example to illustrate why theory translation is non-trivial. Our paper gives a concrete real-world example of issues that arise in translating theory. Our work is also similar to traditional HCI iterative design processes~\cite{buxton2010sketching}, but the critical difference is that past work on iterative design did not consider  theory as an additional source of information. When theory enters the mix, the iterative design process must account for both  concrete user feedback and abstract theoretical considerations. Integrating both concrete and abstract information involves unique challenges, and our paper discusses a method to address these challenges.\\
%Theory translation is also discussed in other disciplines---e.g., implementation science, applied behavioral psychology. Intervention Mapping~\cite{bartholomew1998intervention,kok2004intervention} and Behavior Change Wheels~\cite{michie2008theory,michie2011behaviour} are the two most prominent and well-cited theory translation models. These papers describe how to pick a theory for a specific intervention and implement it in real-world applications. However, most of these real-world applications deal with in-person healthcare services (e.g., visiting a doctor's office) rather than technological interventions. Therefore the only useful part of these models for technological designers is how to choose a theory. Once a theory is chosen, a designer must still fill in all the details to account for theoretical abstractions as we did in our paper.\\
%Since already talked about related work in theory translation in Section~\ref{sec:ttp-general}, we only focus on related work on increasing self-report adherence. Gamification research is closely related to increasing self-report adherence~\cite{van2017gamification}. However, past gamification research did not change virtual reinforcements over time as SARA did~\cite{van2017gamification,werbach2012win,johnson2016gamification}. SARA even went one step further than traditional gamification research: it includes a variety of gamified and non-gamified reinforcements (e.g., life-insights, money) and used theories to justify how to schedule these diverse reinforcements. Another related field is 
